Using RL to Identify Divisive Perspectives Improves LLMs Abilities to Identify Communities on Social Media

The large scale usage of social media, combined with its significant impact, has made it increasingly important to understand it. In particular, identifying user communities, can be helpful for many downstream tasks. However, particularly when models are trained on past data and tested on future, doing this is difficult. In this paper, we hypothesize to take advantage of Large Language Models (LLMs), to better identify user communities. Due to the fact that many LLMs, such as ChatGPT, are fixed and must be treated as black-boxes, we propose an approach to better prompt them, by training a smaller LLM to do this. We devise strategies to train this smaller model, showing how it can improve the larger LLMs ability to detect communities. Experimental results show improvements on Reddit and Twitter data, on the tasks of community detection, bot detection, and news media profiling.

==> extra_results.tex <==


\begin{table*}
\begin{center}
\begin{tabular}{|p{6.4cm}|p{1.4cm}|p{1.4cm}|p{2.4cm}|p{1.4cm}|}
  \hline
  {\textbf{\small Dataset: Model}} & {\textbf{\small Purity}} & {\textbf{\small All Purity}} & {\textbf{\small Purity Num Users}} &  {\textbf{\small F1}} \\

 \hline
 \small Reddit Political: No Focus Areas & \small 67.64 & \small 58.07 & \small 66.19 & \small  \\
 \small Reddit Political: Llama Focus Areas & \small 69.70 & \small 58.20 & \small 68.00 & \small  \\
 \small Reddit Political: Seq2Seq Focus Areas & \small  & \small & \small & \small  \\
 \small Reddit Political: Seq2Seq RL Focus Areas Curr & \small 68.38 & \small 59.21 & \small 66.87 & \small  \\
 \small Reddit Political: Seq2Seq RL Focus Areas Purity & \small 70.83 & \small 58.53 & \small 68.44 & \small  \\
 \hline 
 \small Reddit Economic: No Focus Areas & \small  & \small & \small & \small  \\
 \small Reddit Economic: Llama Focus Areas & \small  & \small & \small & \small  \\
 \small Reddit Economic: Seq2Seq Focus Areas & \small  & \small & \small & \small  \\
 \small Reddit Economic: Seq2Seq RL Focus Areas & \small  & \small & \small & \small  \\
 \hline 
 \small TwiBot: No Focus Areas & \small 46.92 & \small 29.61 & \small 46.43 & \small   \\
 \small TwiBot: Llama Focus Areas & \small  & \small  & \small & \small \\
 \small TwiBot: Seq2Seq Focus Areas & \small  & \small & \small & \small   \\
 \small TwiBot: Seq2Seq RL Focus Areas & \small  & \small & \small & \small   \\
  \hline 

 \hline
\end{tabular}
\end{center}
\captionsetup{justification=centering}
\caption{\small Llama 2 + T5-Large Results}
\label{table:rlhf_results}
\end{table*}

\begin{table*}
\begin{center}
\begin{tabular}{|p{6.4cm}|p{1.4cm}|p{1.4cm}|p{2.4cm}|p{1.3cm}|p{1.3cm}|p{.7cm}|}
  \hline
  {\textbf{\small Dataset: Model}} & {\textbf{\small Purity}} & {\textbf{\small All Purity}} & {\textbf{\small Purity Num Users}} & {\textbf{\small Precision}} & {\textbf{\small Recall}} & {\textbf{\small F1}} \\

 \hline
 \small Reddit Political: No Focus Areas & \small 89.89 & \small 42.01 & \small 76.18 & \small  & & \\
 \small Reddit Political: ChatGPT Focus Areas & \small 84.19 & \small 44.66 & \small 71.64 & \small & &  \\
 \small Reddit Political: Seq2Seq Focus Areas & \small 84.64 & \small 45.48 & \small 72.16 & \small & &  \\
 \small Reddit Political: Seq2Seq RL Focus Areas Curr & \small 83.52 & \small 47.85 & \small 70.36 & \small & &  \\
 \small Reddit Political: Seq2Seq RL Focus Areas Purity & \small 84.50 & \small 44.05 & \small 69.52 & \small & &  \\
 \hline 
 \small Reddit Economic: No Focus Areas & \small  & \small & \small & \small & & \\
 \small Reddit Economic: Llama Focus Areas & \small  & \small & \small & \small & & \\
 \small Reddit Economic: Seq2Seq Focus Areas & \small  & \small & \small & \small & &  \\
 \small Reddit Economic: Seq2Seq RL Focus Areas & \small  & \small & \small & \small & & \\
 \hline 
 \small TwiBot: No Focus Areas & \small  & \small  & \small  & \small & &  \\
 \small TwiBot: Llama Focus Areas & \small & \small & \small & \small & & \\
 \small TwiBot: Seq2Seq Focus Areas & \small  & \small & \small & \small  & & \\
 \small TwiBot: Seq2Seq RL Focus Areas & \small  & \small & \small & \small & &  \\
  \hline 

 \hline
\end{tabular}
\end{center}
\captionsetup{justification=centering}
\caption{\small Chat-GPT + T5-Large Results}
\label{table:chatgpt_rl4f_results}
\end{table*}
